Simulation of left ventricle fluid dynamics with mitral regurgitation from magnetic resonance images with fictitious elastic structure regularization

Computer modeling can provide quantitative insight into cardiac fluid dynamics phenomena that are not evident from standard imaging tools. We propose a new approach to modeling left ventricle fluid dynamics based on an image-driven model-based description of ventricular motion. In this approach, the end-diastolic geometry and time-dependent deformation of the left ventricle cavity are obtained from cardiac magnetic resonance images and a fictitious elastic structure is used to impose the contractile behavior of the left ventricle. This allows seamless treatment of the isovolumic phases. Besides the ventricular motion, the intracavitary fluid dynamics is controlled by the mitral valve. Three different mitral valve models are included in the simulation: an idealized diode (with or without regurgitation) and a lumped parameter model accounting for the opening dynamics of the valve and including regurgitation.

==> conclusions.tex <==
In this work we have presented a methodology for the simulation of LV fluid dynamics. The main features of our technique are (i)~a deformable ellipsoidal geometry for the preliminary description of the LV, (ii)~the combined RBF and trigonometric polynomial interpolations for the reconstruction of the displacement field of the epicardium from MRI data, (iii)~the fictitious linear elastic structure that transfers the interpolated displacement field on the epicardium, and (iv)~the geometrical multiscale method for the implicit coupling of the ventricle with the arterial systemic circulation. The first two ingredients provides a systematic way to set up simulations on an anatomically correct deformable ventricle geometry. The third an automatic way to smooth out the noise and to regularize the imaging data. The last ingredient provides a reliable way to account for the boundary conditions at the ventricle valves and to study the interaction between the ventricular pathologies and the arterial systemic circulation.

Our study has mainly focused on the construction and description of the mathematical multiscale model, while performing some basic calibration and sensitivity analysis of the main parameters. Further analysis should be performed on the sensitivity of the reconstructed LV dynamics on the fictitious elastic structure thickness, which might be adjusted to improve the filtering level of the MRI data noise. Another important aspect regards the modeling of the valve and in particular the correct choice of boundary conditions at the \ThreeD interfaces. The imposition of defective flow rate boundary data at the valve causes strong artifacts and backflow.  A more accurate description of the valve geometry, i.e., the orifice shape and its positioning, is also needed for patient-specific studies, and further validation studies should be performed against in vivo measurements.

The results of the interaction between the \ThreeD LV and the \OneD systemic arterial circulation have made it clear that there is a need for a calibration process to account for the pathological hypertension of the selected patient. This is important not only to recover the correct pressure level in the arteries, but also to obtain more precise estimates of the flow rate wave forms and to highlight the presence of possible backflow. The calibration of the network can be achieved acting on several parameters at the same time, such as the resistances and compliances of the terminals or the elastic and viscoelastic properties of the vessels. However, we have shown that tuning the terminal hydraulic resistances and the reference external pressure of the vessels is enough to recover preliminary reasonable pressure levels.
